Improved approximation for 3-dimensional matching via bounded pathwidth local search

One of the most natural optimization problems is the k-Set Packing problem, where given a family of sets of size at most k one should select a maximum size subfamily of pairwise disjoint sets. A special case of 3-Set Packing is the well known 3-Dimensional Matching problem. Both problems belong to the Karp`s list of 21 NP-complete problems. The best known polynomial time approximation ratio for k-Set Packing is (k + eps)/2 and goes back to the work of Hurkens and Schrijver [SIDMA`89], which gives (1.5 + eps)-approximation for 3-Dimensional Matching. Those results are obtained by a simple local search algorithm, that uses constant size swaps. The main result of the paper is a new approach to local search for k-Set Packing where only a special type of swaps is considered, which we call swaps of bounded pathwidth. We show that for a fixed value of k one can search the space of r-size swaps of constant pathwidth in c^r poly(|F|) time. Moreover we present an analysis proving that a local search maximum with respect to O(log |F|)-size swaps of constant pathwidth yields a polynomial time (k + 1 + eps)/3-approximation algorithm, improving the best known approximation ratio for k-Set Packing. In particular we improve the approximation ratio for 3-Dimensional Matching from 3/2 + eps to 4/3 + eps.

==> fig5.tex <==
\begin{tikzpicture}[scale=0.85]
  \tikzstyle{vertex}=[circle,fill=black,minimum size=0.20cm,inner sep=0pt]
  \tikzstyle{vertex2}=[circle,draw=black,fill=gray!50,minimum size=0.20cm,inner sep=0pt]
 	\tikzstyle{vertex3}=[circle,draw=black,fill=white,minimum size=0.20cm,inner sep=0pt]
 
  \tikzstyle{terminal}=[rectangle,draw=black,fill=white,minimum size=0.2cm,inner sep=0pt]

\node[vertex] (v0) at (0,0){};
\node[vertex] (v1) at (-1,-1){};
\node[vertex] (v2) at (0,-1){};
\node[vertex] (v3) at (1,-1){};


\node[vertex] (v4) at (-1.5,-2){};
\node[vertex] (v5) at (-0.5,-2){};
\node[vertex] (v6) at (0.5,-2){};
\node[vertex] (v7) at (1.5,-2){};

\node[vertex] (v8) at (-2.5,-3){};
\node[vertex] (v9) at (-1.5,-3){};
\node[vertex] (v10) at (-0.5,-3){};
\node[vertex] (v11) at (0.5,-3){};
\node[vertex] (v12) at (1.5,-3){};
\node[vertex] (v13) at (2.5,-3){};

\draw (v1) -- (v0) -- (v2);
\draw (v0) -- (v3);

\draw (v4) -- (v1) -- (v5);
\draw (v6) -- (v2);
\draw (v7) -- (v3);

\draw(v8) -- (v4) -- (v9);
\draw (v10) -- (v5);
\draw (v11) -- (v6) -- (v12);
\draw (v13) -- (v7);

\node[vertex] (x) at (-1.5,-4){};
\draw[dashed] (v8) -- (x) -- (v9);
\draw (x) -- (v10);

\draw[color=gray,line width=2] (v8) -- (v4) -- (v1);
\draw[color=gray,line width=2] (v9) -- (v4);
\draw[color=gray,line width=2] (x) -- (v10) -- (v5) -- (v1);


\end{tikzpicture}

